Differentiable Point-Based Radiance Fields for Efficient View Synthesis

We propose a differentiable rendering algorithm for efficient novel view synthesis. By departing from volume-based representations in favor of a learned point representation, we improve on existing methods more than an order of magnitude in memory and runtime, both in training and inference. The method begins with a uniformly-sampled random point cloud and learns per-point position and view-dependent appearance, using a differentiable splat-based renderer to evolve the model to match a set of input images. Our method is up to 300x faster than NeRF in both training and inference, with only a marginal sacrifice in quality, while using less than 10~MB of memory for a static scene. For dynamic scenes, our method trains two orders of magnitude faster than STNeRF and renders at near interactive rate, while maintaining high image quality and temporal coherence even without imposing any temporal-coherency regularizers.

==> 4_implementation.tex <==
% \subsection{Software} We implemented everything in MATLAB. For a 25 megapixel image, the algorithm takes 10~secs to converge in 500~iterations; we show convergence in Figure~\ref{fig:convergence}. We hand-tuned the parameters to $\lambda_1=0.001$ and $\sigma=12.45$. All source code and data will be made available (\emph{this addresses the reproducibility issue}).  


% \subsection{Hardware} We built a really cool prototype. Now list all the prototype parts and specific model numbers. The hardware should be fully reproducible from the information given here! You can see a photograph of the prototype in Figure~\ref{fig:prototype}. 


% \subsection{Calibration} Describe in detail how you calibrated the hardware setup!


% \begin{figure}
% 	\centering
% 		\includegraphics[width=\columnwidth]{figures/convergence}
% 		\caption{convergence - should go down.}
% 		\label{fig:convergence}
% \end{figure}

% \begin{figure}
% 	\centering
% 		\includegraphics[width=\columnwidth]{figures/prototype}
% 		\caption{Show photo of prototype and label parts.}
% 		\label{fig:prototype}
% \end{figure}

==> 5_results_bak.tex <==
% \subsection{Analysis}

% Evaluate all algorithmic or hardware parameters here.

% \begin{figure}[t]
% 	\centering
% 		\includegraphics[width=\columnwidth]{figures/analysis.png}
% 		\caption{Show some plot that shows that the effects of the parameters are.}
% 		\label{fig:analysis}
% \end{figure}

% \subsection{Interpretation}

% Potentially analysis your decompositions, patterns, or whatever you do and try to make them intuitive. What does this complicated algorithm do intuitively?


% \subsection{Results}

% Show visually compelling results here. Make sure you show different results, i.e. if you have multiple scenes make sure that every scene or result tells its own story!

% \begin{figure*}[t]
% 	\centering
% 		\includegraphics[width=\textwidth]{figures/results.png}
% 		\caption{Show results for multiple examples here. Each one should tell a different story!}
% 		\label{fig:results}
% \end{figure*}

% \subsection{Comparison to Previous Work}

% You need both qualitative and quantitative comparisons. The qualitative comparison must be absolutely and unmistabably obvious! If it's hard to see, zoom in and magnify what they are supposed to look at. 

% \begin{figure}[t]
% 	\centering
% 		\includegraphics[width=\columnwidth]{figures/comparison.png}
% 		\caption{This has to be absolutely obvious!}
% 		\label{fig:comparison}
% \end{figure}

% \begin{figure*}[t]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=1.0\linewidth]{figures/result.JPG}
%   \caption{\textbf{Qualitatively experiment result.} Here we show depth image, the rendered rgb image and the ground-truth reference image. From top to bottom, the objects are chair, drums, ficus and hotdog.}
%   \label{fig:result}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=1.0\linewidth]{figures/ablation.JPG}
%   \caption{\textbf{Ablation study for different modules.} The images from left to right are: 1. Optimizing only via diffuse color, 2. Joint optimization for both the point position and the diffuse color, 3. Joint optimization with consistency filter function, 4. Image translation refinement.}
%   \label{fig:ablation}
% \end{figure*}

We implement our model with pytorch and pytorch3d, on one Nvidia P100 GPU. We choose nerf synthetic dataset as the benchmark, which contains eight different objects. For each object, there are 100 training images, 15 validation images and 23 test images. For all the images, the camera parameters are known. As for the training setup, here we use non-synchronous learning strategy for optimizing the point position and texture, to be specific, the initial learning rate for neural brdf model and the left part are $3e-3$ and $8e-4$ respectively. Both of them are exponentially decayed for every epoch (20 epochs in total) with a factor of $0.93$. $\lambda$ equals to $0.06$.


\subsection{Baseline Introduction}
Here we choose the nerf\cite{mildenhall2020nerf} model as the first baseline. There are also a brunch of previous works which take the extra estimated geometry information as input. On the contrary, our experiment setup is exactly the same as nerf and there is no extra geometry information as the input. Consequently, we only compare with those who has no extra geometry data either. Here, we choose the multi-view-stereo nerf\cite{chen2021mvsnerf}, which is pretrained on a large scale extra dataset for novel view synthesis. The major advantage for this work is that it can be fast deployed to a new dataset after a fast finetuning stage. 



\subsection{Rendering Comparison}
We use two metrics to measure the rendering quality: PSNR and SSIM, just as many previous work does. As shown in Tab.\ref{tab:result}, we compare our method with two baselines. It is clear to see that our model performs better in most objects than the MVSnerf baseline and can achieve comparable performance with Nerf baseline. Qualitatively, we also visualize some rendering images for comparison. Although there is no geometry as the input, our model can estimate the geometry information such as depth map. The results are shown in Fig\ref{fig:result}. 

We use the training time and inference time to measure the convergence speed and rendering speed, just as shown in Tab\ref{tab:result_time}. The Mvsnerf baseline requires extra pretraining, which takes about 45 hours on one single P100 GPU. On the contrary, our model and nerf baseline does not. As for the training time, we measure the average time of all eight different object datasets. It is clear to see that our model only takes about 8 min per object, which is around one third of mvsnerf finetuning time. For comparison, nerf takes about 128 hours, which is more than 150x longer than ours. As for the inference time, we measure the average time of rendering one single image, mvsnerf inference time is longer than nerf baseline, 12s per image. However, for our model, it is 100x faster than these two baselines, we can rendering one single image within 0.11s with one single P100 GPU.



\begin{table}
\centering
    \begin{tabular}{llll}
    \toprule
    Method    & Pretraining   & Training & Test  \\ \cline{1-4}
    Ours      & Not required  & 8min        & 0.11s  \\ \cline{1-4}
    Mvsnerf-w & Required(45h) & 22min         & \textgreater{}12s   \\ \cline{1-4}
    Nerf      & Not required  & 16.5h          & 12s \\
    \bottomrule
    \end{tabular}
\caption{\textbf{Model training and inference time comparison} Here we compare the training and inference time for the baselines and our model. The training time is counted on the average time on eight different object in the nerf synthetic time on one single gpu. The inference time is counted as rendering one image on one single gpu. }
\label{tab:result_time}
\end{table}


% \begin{figure}[t]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.6\linewidth}{0pt}}
%   \includegraphics[width=0.95\linewidth]{images/depthimg.JPG}
%   \caption{\textbf{Depth estimation visualizations.} The first row is from the ground-truth reference image and the second row is our rendered depth image. }
%   \label{fig:depth}
% \end{figure}



\subsection{Ablation Study}
To prove the effectiveness of each module, we here provide some ablation studies.

We first visualize the effectiveness of some modules in Fig\ref{fig:ablation}. From left to right, they are rendering results from: 1. Only use diffuse color as the learnable parameters and fix the initalized point cloud. The quantitative performance (PSNR value) for this ablation experiment is only about 23.4 dB, which is much less than our full model, 27.79 dB. 2. Joint optimization for both diffuse color and the point position without repeating applying the filter function. 3. Joint optimization with repeated filter function. 4. The rendering result after image refinement module. 5. the ground truth reference image.

The effectiveness of the learnable spherical harmonics is shown in Fig\ref{fig:sh}. The left two images are from the ground-truth reference images, the middle part are the model output without spherical harmonics, and the right one are with spherical harmonics(n=9). It is clear to see that this spherical harmonics enables modeling the view-dependent effect.

The effectiveness of total variance regularizer and image translation refinement module is shown in Tab\ref{tab:ablation2}. The total variance loss can help boost the performance about 0.4 dB and the image translation module can help improve about 1.2 dB.



\begin{table}
\centering
\begin{tabular}{lccc}
\toprule
Ablations   & PSNR$\uparrow$  & SSIM $\uparrow$ & LPIPS $\downarrow$\\ \hline
Ours-full   & 27.79 & 0.946    & 0.124     \\ \hline
Ours-w/o sh & 26.82 & 0.934    & 0.132     \\ \hline
Ours-w/o g  & 26.53 & 0.926    & 0.137     \\ \hline
Ours-w/o tv & 27.41 & 0.941    & 0.129     \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Ablation studies.} From top to bottom, they are full model, without spherical harmonics, without image translation module, without total variance loss.}
\label{tab:ablation2}
\end{table}


% \begin{figure}[]
%   \centering
% %   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=1.0\linewidth]{figures/sh.JPG}
%   \caption{\textbf{Ablation study for the spherical harmonics.}The top row and the bottom row are from the training set and the test set respectively. From left to right, they are ground-truth image, our model without spherical harmonics and ours with 9 harmonics.}
%   \label{fig:sh}
% \end{figure}

\subsection{Other necessary visualizations}
Our motivation comes from the question whether nerf model learns the multi-view color consistency. To answer this question, we design the nerf silhousette exploration experiment: replacing the nerf rgb image with the corresponding silhousette mask. Here we show the result for this experiment in Fig\ref{fig:mask}. It is clear to see that nerf model can render the silhousette mask pretty well after training in the new setting. Since there is no multi-view geometry consistency information as the input, It is purely learnt from the pixel itself, rather than the local feature. This leads to the thinking of visual convex hull initialization.

Another visualization we post here is the soft multi-view consistency filter function. The usage for this soft filter function is to extend our model to forwardfacing dataset in which the scene mask is not easy to obtain. We also randomly sample the points in the space and then project them into all the training images, which means there is one color set for each point. Rather than compute the sum of mask value, we compute the variance of the colors and filter out the points whose variance is large than a certain threshold. We visualize the variance slice images from different depth levels (the depth relative to one specific reference image) in Fig\ref{fig:depthvar}. It is clear to see that this variance figures can estimate the geometry to some extent. This means that our model can be extended to the non-central dataset.


==> 6_bellsnwhistles.tex <==
% Mandatory video to watch on youtube: shamwow (\url{https://www.youtube.com/watch?v=QwRISkyV_B8}).

% Now that we have focused on introducing method~D, deriving a bunch of math, analyzing all the algorithmic parameters, comparing it to previous work, and showing a whole lot of really cool results for the core thing that this paper is focused on, let us show you a bunch of extra stuff that you can also do with the proposed approach.

% Remember the shamwow video. This is basically a wiping cloth and for the past couple of minutes in the video clip (or the last 3 sections of the paper), we have focused on the main application: wiping stuff off all possibly conceivable surfaces. But now we'll show you a bunch of other stuff that you get for free! For example, you can use shamwow as a mop (wiping cloth with a stick) so you can clean your entire house, you can also use shamwow for wiping your cat or dog or your bird, you can clean your car, and finally, you can also use it as a diaper and as a blanket. 

% Be concise in this section, because the paper is about the previous 3 sections. Just write a few paragraphs and show the best results for each bell \& whistle.




==> 7_discussion.tex <==
% In summary, we proposed a new thing, analyzed it in detail, showed a bunch of results, built a prototype, etc etc. Basically write a paragraph summarizing the paper. By now the reader may be asleep and they probably missed a couple of important details when they skimmed over the technical sections, so just briefly summarize everything in one paragraph. 

% Make sure to highlight all the benefits of your approach in this summary! You can even write a second paragraph just discussing these.

% \paragraph{Limitations} However, as with all methods, since there would never be any future papers in this area, our method also has limitations. First, our approach makes the following fundamental assumptions ... If these assumptions are not valid, as is the case in scenarios~x,~y, and~z, then this method may not work. Second, our methods also fails in the following scenarios: ... An example of \emph{how} it fails is shown in Figure~\ref{fig:failure}. 

% \begin{figure}
% 	\centering
% 		\includegraphics[width=\columnwidth]{figures/failure.png}
% 		\caption{Failure case. Don't just show that it fails here but \emph{how it fails!}}
% 		\label{fig:failure}
% \end{figure}


% Now discuss a few possible strategies for overcoming these limitations here (or just integrate them into the previous paragraph so as to dismiss the limitations as easily fixable). But focus on possible methods to fix exactly what's wrong with your current approach.

% \paragraph{Future Work} In the future, we will actually fix all the things that currently don't work. We would also like to apply the approach proposed here to the completely different problem of ... we believe this has a lot of promise. And we want to do a bunch of other stuff as well.
  

 

